SN 2017gmr: An energetic Type II-P supernova with asymmetries

We present high-cadence ultraviolet (UV), optical, and near-infrared (NIR) data on the luminous Type II-P supernova SN 2017gmr from hours after discovery through the first 180 days. SN 2017gmr does not show signs of narrow, high-ionization emission lines in the early optical spectra, yet the optical lightcurve evolution suggests that an extra energy source from circumstellar medium (CSM) interaction must be present for at least 2 days after explosion. Modeling of the early lightcurve indicates a ~500R$_{\odot}$ progenitor radius, consistent with a rather compact red supergiant, and late-time luminosities indicate up to 0.130 $\pm$ 0.026 M$_{\odot}$ of $^{56}$Ni are present, if the lightcurve is solely powered by radioactive decay, although the $^{56}$Ni mass may be lower if CSM interaction contributes to the post-plateau luminosity. Prominent multi-peaked emission lines of H$\alpha$ and [O I] emerge after day 154, as a result of either an asymmetric explosion or asymmetries in the CSM. The lack of narrow lines within the first two days of explosion in the likely presence of CSM interaction may be an example of close, dense, asymmetric CSM that is quickly enveloped by the spherical supernova ejecta.

==> opt_phot_table.tex <==
\startlongtable
\begin{deluxetable}{lcccc}%[!t]
\tablecaption{SN~2017gmr Optical Photometry \label{tab:optphot}}
\tablehead{\colhead{MJD} & \colhead{Phase } & \colhead{Magnitude} & \colhead{Error} & \colhead{Telescope} \\
}
\startdata
\multicolumn{5}{c}{$U$}\\
\hline 
58000.276 & +1.19 & 14.44 & 0.05 & LCOGT-1m \\
58000.280 & +0.077 & 14.37 & 0.04 & LCOGT-1m \\
58000.358 & +0.16 & 14.11 & 0.02 & LCOGT-1m \\
58000.362 & +0.16 & 14.11 & 0.02 & LCOGT-1m \\
58000.631 & +0.43 & 13.90 & 0.03 & LCOGT-1m \\
58000.635 & +0.43 & 13.90 & 0.03 & LCOGT-1m \\
58000.984 & +0.78 & 13.87 & 0.05 & LCOGT-1m \\
58000.987 & +0.78 & 13.94 & 0.03 & LCOGT-1m \\
58001.115 & +0.91 & 13.89 & 0.03 & LCOGT-1m \\
58001.119 & +0.92 & 13.91 & 0.03 & LCOGT-1m \\
58001.597 & +1.4 & 14.07 & 0.04 & LCOGT-1m \\
58001.601 & +1.4 & 13.99 & 0.03 & LCOGT-1m \\
58001.726 & +1.5 & 14.00 & 0.02 & LCOGT-1m \\
58001.730 & +1.5 & 13.99 & 0.02 & LCOGT-1m \\
58002.229 & +2.0 & 14.06 & 0.03 & LCOGT-1m \\
58002.233 & +2.0 & 13.98 & 0.02 & LCOGT-1m \\
58002.660 & +2.5 & 14.00 & 0.03 & LCOGT-1m \\
58002.664 & +2.5 & 14.00 & 0.03 & LCOGT-1m \\
58002.991 & +2.8 & 13.97 & 0.02 & LCOGT-1m \\
58002.995 & +2.8 & 13.96 & 0.02 & LCOGT-1m \\
58003.266 & +3.1 & 13.99 & 0.02 & LCOGT-1m \\
58003.269 & +3.1 & 13.96 & 0.02 & LCOGT-1m \\
58003.592 & +3.4 & 13.95 & 0.03 & LCOGT-1m \\
58003.596 & +3.4 & 14.04 & 0.04 & LCOGT-1m \\
58003.990 & +3.8 & 13.93 & 0.03 & LCOGT-1m \\
58003.994 & +3.8 & 13.94 & 0.03 & LCOGT-1m \\
58004.318 & +4.1 & 13.92 & 0.02 & LCOGT-1m \\
58004.322 & +4.1 & 13.95 & 0.02 & LCOGT-1m \\
58004.661 & +4.5 & 13.95 & 0.03 & LCOGT-1m \\
58004.665 & +4.5 & 13.92 & 0.03 & LCOGT-1m \\
58005.114 & +4.9 & 13.90 & 0.02 & LCOGT-1m \\
58005.118 & +4.9 & 13.88 & 0.02 & LCOGT-1m \\
58010.751 & +10.5 & 14.00 & 0.03 & LCOGT-1m \\
58010.755 & +10.6 & 14.02 & 0.03 & LCOGT-1m \\
58011.767 & +11.6 & 14.04 & 0.02 & LCOGT-1m \\
58011.771 & +11.6 & 14.04 & 0.02 & LCOGT-1m \\
58013.732 & +13.5 & 14.07 & 0.02 & LCOGT-1m \\
58013.736 & +13.5 & 14.06 & 0.02 & LCOGT-1m \\
58014.990 & +14.8 & 14.23 & 0.02 & LCOGT-1m \\
58014.994 & +14.8 & 14.19 & 0.02 & LCOGT-1m \\
58015.734 & +15.5 & 14.21 & 0.02 & LCOGT-1m \\
58015.738 & +15.5 & 14.21 & 0.02 & LCOGT-1m \\
58016.556 & +16.4 & 14.23 & 0.02 & LCOGT-1m \\
58016.560 & +16.4 & 14.26 & 0.02 & LCOGT-1m \\
58019.948 & +19.7 & 14.40 & 0.02 & LCOGT-1m \\
58019.952 & +19.7 & 14.41 & 0.02 & LCOGT-1m \\
58021.122 & +20.9 & 14.54 & 0.02 & LCOGT-1m \\
58021.125 & +20.9 & 14.53 & 0.02 & LCOGT-1m \\
58024.938 & +24.7 & 14.86 & 0.02 & LCOGT-1m \\
58024.941 & +24.7 & 14.86 & 0.02 & LCOGT-1m \\
58028.893 & +28.7 & 15.40 & 0.07 & LCOGT-1m \\
58029.037 & +28.8 & 15.32 & 0.07 & LCOGT-1m \\
58029.165 & +29.0 & 15.34 & 0.03 & LCOGT-1m \\
58029.168 & +29.0 & 15.30 & 0.03 & LCOGT-1m \\
58032.663 & +32.5 & 15.70 & 0.05 & LCOGT-1m \\
58032.666 & +32.5 & 15.76 & 0.06 & LCOGT-1m \\
58035.326 & +35.1 & 15.79 & 0.03 & LCOGT-1m \\
58035.329 & +35.1 & 15.74 & 0.03 & LCOGT-1m \\
58039.333 & +39.1 & 15.94 & 0.04 & LCOGT-1m \\
58039.335 & +39.1 & 15.96 & 0.04 & LCOGT-1m \\
58046.253 & +46.0 & 16.30 & 0.03 & LCOGT-1m \\
58046.257 & +46.1 & 16.30 & 0.03 & LCOGT-1m \\
58047.170 & +47.0 & 16.44 & 0.03 & LCOGT-1m \\
58047.212 & +47.0 & 16.38 & 0.02 & LCOGT-1m \\
58047.216 & +47.0 & 16.41 & 0.02 & LCOGT-1m \\
58047.254 & +47.1 & 16.49 & 0.03 & LCOGT-1m \\
58047.257 & +47.1 & 16.50 & 0.03 & LCOGT-1m \\
58047.304 & +47.1 & 16.45 & 0.03 & LCOGT-1m \\
58047.308 & +47.1 & 16.50 & 0.03 & LCOGT-1m \\
58048.645 & +48.4 & 16.47 & 0.03 & LCOGT-1m \\
58048.649 & +48.4 & 16.45 & 0.03 & LCOGT-1m \\
58052.853 & +52.6 & 16.70 & 0.03 & LCOGT-1m \\
58052.857 & +52.7 & 16.65 & 0.03 & LCOGT-1m \\
58057.204 & +57.0 & 16.92 & 0.03 & LCOGT-1m \\
58057.208 & +57.0 & 16.93 & 0.03 & LCOGT-1m \\
58062.018 & +61.8 & 17.14 & 0.06 & LCOGT-1m \\
58062.022 & +61.8 & 17.27 & 0.06 & LCOGT-1m \\
\hline 
\multicolumn{5}{c}{$B$}\\
\hline 
58000.284 & +0.081 & 15.13 & 0.02 & LCOGT-1m \\
58000.287 & +0.084 & 15.15 & 0.02 & LCOGT-1m \\
58000.366 & +0.16 & 14.97 & 0.01 & LCOGT-1m \\
58000.369 & +0.17 & 14.98 & 0.01 & LCOGT-1m \\
58000.639 & +0.44 & 14.78 & 0.02 & LCOGT-1m \\
58000.642 & +0.44 & 14.79 & 0.02 & LCOGT-1m \\
58000.992 & +0.79 & 14.74 & 0.02 & LCOGT-1m \\
58000.994 & +0.79 & 14.68 & 0.02 & LCOGT-1m \\
58001.000 & +0.80 & 14.60 & 0.09 & Konkoly \\
58001.123 & +0.92 & 14.70 & 0.02 & LCOGT-1m \\
58001.125 & +0.92 & 14.71 & 0.02 & LCOGT-1m \\
58001.606 & +1.4 & 14.80 & 0.02 & LCOGT-1m \\
58001.608 & +1.4 & 14.79 & 0.02 & LCOGT-1m \\
58001.734 & +1.5 & 14.76 & 0.02 & LCOGT-1m \\
58001.737 & +1.5 & 14.73 & 0.02 & LCOGT-1m \\
58002.237 & +2.0 & 14.70 & 0.02 & LCOGT-1m \\
58002.240 & +2.0 & 14.76 & 0.02 & LCOGT-1m \\
58002.668 & +2.5 & 14.74 & 0.02 & LCOGT-1m \\
58002.670 & +2.5 & 14.71 & 0.02 & LCOGT-1m \\
58002.999 & +2.8 & 14.65 & 0.02 & LCOGT-1m \\
58003.002 & +2.8 & 14.65 & 0.02 & LCOGT-1m \\
58003.274 & +3.1 & 14.68 & 0.01 & LCOGT-1m \\
58003.276 & +3.1 & 14.69 & 0.01 & LCOGT-1m \\
58003.600 & +3.4 & 14.76 & 0.03 & LCOGT-1m \\
58003.603 & +3.4 & 14.75 & 0.03 & LCOGT-1m \\
58003.998 & +3.8 & 14.63 & 0.02 & LCOGT-1m \\
58004.001 & +3.8 & 14.63 & 0.02 & LCOGT-1m \\
58004.080 & +3.9 & 14.47 & 0.08 & Konkoly \\
58004.329 & +4.1 & 14.68 & 0.02 & LCOGT-1m \\
58004.669 & +4.5 & 14.67 & 0.02 & LCOGT-1m \\
58004.672 & +4.5 & 14.68 & 0.02 & LCOGT-1m \\
58005.080 & +4.9 & 14.47 & 0.09 & Konkoly \\
58005.122 & +4.9 & 14.61 & 0.02 & LCOGT-1m \\
58005.125 & +4.9 & 14.59 & 0.01 & LCOGT-1m \\
58010.759 & +10.6 & 14.66 & 0.02 & LCOGT-1m \\
58010.762 & +10.6 & 14.65 & 0.02 & LCOGT-1m \\
58011.600 & +11.4 & 14.64 & 0.08 & NOT \\
58011.775 & +11.6 & 14.67 & 0.01 & LCOGT-1m \\
58011.778 & +11.6 & 14.66 & 0.01 & LCOGT-1m \\
58013.740 & +13.5 & 14.68 & 0.01 & LCOGT-1m \\
58013.742 & +13.5 & 14.69 & 0.01 & LCOGT-1m \\
58014.700 & +14.5 & 14.69 & 0.05 & NOT \\
58014.998 & +14.8 & 14.67 & 0.01 & LCOGT-1m \\
58015.001 & +14.8 & 14.68 & 0.01 & LCOGT-1m \\
58015.742 & +15.5 & 14.74 & 0.01 & LCOGT-1m \\
58015.745 & +15.5 & 14.72 & 0.01 & LCOGT-1m \\
58016.564 & +16.4 & 14.80 & 0.01 & LCOGT-1m \\
58016.567 & +16.4 & 14.82 & 0.01 & LCOGT-1m \\
58017.550 & +17.3 & 14.72 & 0.02 & NOT \\
58019.300 & +19.1 & 14.83 & 0.08 & SLOTIS \\
58019.956 & +19.8 & 14.80 & 0.01 & LCOGT-1m \\
58019.958 & +19.8 & 14.78 & 0.01 & LCOGT-1m \\
58021.128 & +20.9 & 14.87 & 0.01 & LCOGT-1m \\
58021.129 & +20.9 & 14.86 & 0.01 & LCOGT-1m \\
58021.300 & +21.1 & 14.89 & 0.08 & SLOTIS \\
58022.300 & +22.1 & 14.89 & 0.08 & SLOTIS \\
58023.510 & +23.3 & 14.94 & 0.04 & NOT \\
58024.944 & +24.7 & 14.99 & 0.01 & LCOGT-1m \\
58024.945 & +24.7 & 14.99 & 0.01 & LCOGT-1m \\
58025.300 & +25.1 & 15.00 & 0.07 & SLOTIS \\
58028.500 & +28.3 & 15.01 & 0.11 & Liverpool \\
58029.171 & +29.0 & 15.21 & 0.02 & LCOGT-1m \\
58029.173 & +29.0 & 15.20 & 0.02 & LCOGT-1m \\
58032.300 & +32.1 & 15.21 & 0.08 & SLOTIS \\
58032.669 & +32.5 & 15.34 & 0.03 & LCOGT-1m \\
58032.670 & +32.5 & 15.45 & 0.04 & LCOGT-1m \\
58034.550 & +34.3 & 15.23 & 0.07 & Liverpool \\
58035.332 & +35.1 & 15.36 & 0.02 & LCOGT-1m \\
58035.333 & +35.1 & 15.37 & 0.02 & LCOGT-1m \\
58036.620 & +36.4 & 15.31 & 0.13 & NOT \\
58038.300 & +38.1 & 15.35 & 0.09 & SLOTIS \\
58039.338 & +39.1 & 15.46 & 0.01 & LCOGT-1m \\
58039.340 & +39.1 & 15.48 & 0.01 & LCOGT-1m \\
58041.300 & +41.1 & 15.42 & 0.09 & SLOTIS \\
58043.600 & +43.4 & 15.42 & 0.06 & Liverpool \\
58046.261 & +46.1 & 15.62 & 0.01 & LCOGT-1m \\
58046.264 & +46.1 & 15.60 & 0.01 & LCOGT-1m \\
58047.220 & +47.0 & 15.61 & 0.01 & LCOGT-1m \\
58047.223 & +47.0 & 15.60 & 0.01 & LCOGT-1m \\
58047.312 & +47.1 & 15.64 & 0.01 & LCOGT-1m \\
58047.314 & +47.1 & 15.63 & 0.01 & LCOGT-1m \\
58047.600 & +47.4 & 15.54 & 0.04 & NOT \\
58048.449 & +48.2 & 15.45 & 0.07 & Liverpool \\
58048.653 & +48.4 & 15.69 & 0.01 & LCOGT-1m \\
58048.655 & +48.5 & 15.70 & 0.01 & LCOGT-1m \\
58049.300 & +49.1 & 15.55 & 0.09 & SLOTIS \\
58051.560 & +51.4 & 15.65 & 0.02 & NOT \\
58052.861 & +52.7 & 15.74 & 0.01 & LCOGT-1m \\
58052.863 & +52.7 & 15.74 & 0.01 & LCOGT-1m \\
58053.200 & +53.0 & 15.61 & 0.05 & SLOTIS \\
58057.212 & +57.0 & 15.92 & 0.01 & LCOGT-1m \\
58057.215 & +57.0 & 15.93 & 0.01 & LCOGT-1m \\
58058.400 & +58.2 & 15.63 & 0.12 & Liverpool \\
58062.026 & +61.8 & 16.01 & 0.02 & LCOGT-1m \\
58062.029 & +61.8 & 15.97 & 0.02 & LCOGT-1m \\
58066.580 & +66.4 & 15.95 & 0.04 & NOT \\
58067.157 & +67.0 & 16.13 & 0.01 & LCOGT-1m \\
58067.159 & +67.0 & 16.13 & 0.01 & LCOGT-1m \\
58072.400 & +72.2 & 16.00 & 0.07 & Liverpool \\
58073.018 & +72.8 & 16.17 & 0.02 & LCOGT-1m \\
58073.020 & +72.8 & 16.17 & 0.02 & LCOGT-1m \\
58074.200 & +74.0 & 16.05 & 0.06 & SLOTIS \\
58077.200 & +77.0 & 16.12 & 0.08 & SLOTIS \\
58077.490 & +77.3 & 16.20 & 0.10 & Liverpool \\
58080.200 & +80.0 & 16.24 & 0.05 & SLOTIS \\
58080.549 & +80.3 & 16.54 & 0.02 & LCOGT-1m \\
58080.552 & +80.3 & 16.48 & 0.02 & LCOGT-1m \\
58083.200 & +83.0 & 16.40 & 0.06 & SLOTIS \\
58084.200 & +84.0 & 16.51 & 0.13 & Asiago-Schmidt \\
58087.072 & +86.9 & 16.78 & 0.02 & LCOGT-1m \\
58087.075 & +86.9 & 16.79 & 0.02 & LCOGT-1m \\
58089.809 & +89.6 & 17.07 & 0.04 & LCOGT-1m \\
58089.812 & +89.6 & 17.11 & 0.04 & LCOGT-1m \\
58090.800 & +90.6 & 17.00 & 0.10 & Asiago-Schmidt \\
58090.826 & +90.6 & 17.16 & 0.03 & LCOGT-1m \\
58090.829 & +90.6 & 17.18 & 0.03 & LCOGT-1m \\
58091.862 & +91.7 & 17.20 & 0.03 & LCOGT-1m \\
58091.865 & +91.7 & 17.20 & 0.02 & LCOGT-1m \\
58093.540 & +93.3 & 17.18 & 0.02 & NOT \\
58093.834 & +93.6 & 17.41 & 0.02 & LCOGT-1m \\
58093.836 & +93.6 & 17.33 & 0.02 & LCOGT-1m \\
58095.815 & +95.6 & 17.47 & 0.02 & LCOGT-1m \\
58095.817 & +95.6 & 17.47 & 0.02 & LCOGT-1m \\
58096.390 & +96.2 & 17.36 & 0.09 & Asiago-Schmidt \\
58096.800 & +96.6 & 17.53 & 0.03 & LCOGT-1m \\
58096.803 & +96.6 & 17.55 & 0.02 & LCOGT-1m \\
58097.149 & +96.9 & 17.57 & 0.02 & LCOGT-1m \\
58097.152 & +96.9 & 17.59 & 0.02 & LCOGT-1m \\
58099.225 & +99.0 & 17.72 & 0.09 & LCOGT-1m \\
58101.181 & +101.0 & 17.73 & 0.02 & LCOGT-1m \\
58101.184 & +101.0 & 17.76 & 0.02 & LCOGT-1m \\
58102.063 & +101.9 & 17.74 & 0.02 & LCOGT-1m \\
58102.066 & +101.9 & 17.73 & 0.02 & LCOGT-1m \\
58103.148 & +102.9 & 17.90 & 0.02 & LCOGT-1m \\
58103.151 & +102.9 & 17.94 & 0.02 & LCOGT-1m \\
58103.200 & +103.0 & 17.63 & 0.08 & SLOTIS \\
58104.177 & +104.0 & 17.94 & 0.02 & LCOGT-1m \\
58104.180 & +104.0 & 17.92 & 0.02 & LCOGT-1m \\
58104.400 & +104.2 & 17.61 & 0.11 & Liverpool \\
58105.280 & +105.1 & 17.78 & 0.12 & Asiago-Schmidt \\
58105.816 & +105.6 & 17.88 & 0.03 & LCOGT-1m \\
58105.820 & +105.6 & 17.88 & 0.03 & LCOGT-1m \\
58106.200 & +106.0 & 17.70 & 0.08 & SLOTIS \\
58109.340 & +109.1 & 17.87 & 0.12 & Liverpool \\
58109.340 & +109.1 & 17.87 & 0.12 & Asiago-Schmidt \\
58112.200 & +112.0 & 17.79 & 0.10 & SLOTIS \\
58113.854 & +113.7 & 18.09 & 0.02 & LCOGT-1m \\
58113.859 & +113.7 & 18.11 & 0.02 & LCOGT-1m \\
58114.430 & +114.2 & 17.81 & 0.11 & Liverpool \\
58121.859 & +121.7 & 18.17 & 0.03 & LCOGT-1m \\
58121.863 & +121.7 & 18.22 & 0.03 & LCOGT-1m \\
58129.827 & +129.6 & 18.26 & 0.02 & LCOGT-1m \\
58129.831 & +129.6 & 18.27 & 0.02 & LCOGT-1m \\
58137.380 & +137.2 & 18.17 & 0.02 & NOT \\
58139.077 & +138.9 & 18.23 & 0.02 & LCOGT-1m \\
58139.081 & +138.9 & 18.25 & 0.02 & LCOGT-1m \\
58147.431 & +147.2 & 18.51 & 0.04 & LCOGT-1m \\
58147.435 & +147.2 & 18.40 & 0.04 & LCOGT-1m \\
58149.042 & +148.8 & 18.39 & 0.05 & LCOGT-1m \\
58149.046 & +148.8 & 18.29 & 0.06 & LCOGT-1m \\
58156.417 & +156.2 & 18.52 & 0.04 & LCOGT-1m \\
58156.421 & +156.2 & 18.50 & 0.03 & LCOGT-1m \\
58163.340 & +163.1 & 18.37 & 0.03 & NOT \\
58164.018 & +163.8 & 18.43 & 0.06 & LCOGT-1m \\
58164.022 & +163.8 & 18.57 & 0.04 & LCOGT-1m \\
58172.012 & +171.8 & 18.37 & 0.07 & LCOGT-1m \\
58172.016 & +171.8 & 18.49 & 0.06 & LCOGT-1m \\
58173.018 & +172.8 & 18.43 & 0.08 & LCOGT-1m \\
58174.765 & +174.6 & 18.50 & 0.07 & LCOGT-1m \\
58174.768 & +174.6 & 18.52 & 0.07 & LCOGT-1m \\
58176.764 & +176.6 & 18.61 & 0.05 & LCOGT-1m \\
58176.768 & +176.6 & 18.63 & 0.05 & LCOGT-1m \\
\hline 
\multicolumn{5}{c}{$V$}\\
\hline 
58000.290 & +0.087 & 14.93 & 0.01 & LCOGT-1m \\
58000.292 & +0.089 & 14.91 & 0.01 & LCOGT-1m \\
58000.372 & +0.17 & 14.87 & 0.01 & LCOGT-1m \\
58000.374 & +0.17 & 14.87 & 0.01 & LCOGT-1m \\
58000.645 & +0.44 & 14.62 & 0.02 & LCOGT-1m \\
58000.646 & +0.44 & 14.65 & 0.02 & LCOGT-1m \\
58000.997 & +0.79 & 14.52 & 0.02 & LCOGT-1m \\
58000.999 & +0.80 & 14.53 & 0.02 & LCOGT-1m \\
58001.000 & +0.80 & 14.57 & 0.08 & Konkoly \\
58001.128 & +0.93 & 14.54 & 0.02 & LCOGT-1m \\
58001.130 & +0.93 & 14.56 & 0.02 & LCOGT-1m \\
58001.611 & +1.4 & 14.62 & 0.02 & LCOGT-1m \\
58001.612 & +1.4 & 14.59 & 0.02 & LCOGT-1m \\
58001.740 & +1.5 & 14.58 & 0.01 & LCOGT-1m \\
58001.741 & +1.5 & 14.58 & 0.01 & LCOGT-1m \\
58002.243 & +2.0 & 14.52 & 0.02 & LCOGT-1m \\
58002.244 & +2.0 & 14.52 & 0.02 & LCOGT-1m \\
58002.673 & +2.5 & 14.47 & 0.01 & LCOGT-1m \\
58002.675 & +2.5 & 14.48 & 0.01 & LCOGT-1m \\
58003.005 & +2.8 & 14.43 & 0.01 & LCOGT-1m \\
58003.006 & +2.8 & 14.44 & 0.01 & LCOGT-1m \\
58003.279 & +3.1 & 14.47 & 0.01 & LCOGT-1m \\
58003.280 & +3.1 & 14.46 & 0.01 & LCOGT-1m \\
58003.605 & +3.4 & 14.40 & 0.02 & LCOGT-1m \\
58003.607 & +3.4 & 14.37 & 0.02 & LCOGT-1m \\
58004.004 & +3.8 & 14.39 & 0.02 & LCOGT-1m \\
58004.005 & +3.8 & 14.37 & 0.02 & LCOGT-1m \\
58004.080 & +3.9 & 14.37 & 0.07 & Konkoly \\
58004.331 & +4.1 & 14.42 & 0.01 & LCOGT-1m \\
58004.333 & +4.1 & 14.41 & 0.01 & LCOGT-1m \\
58004.674 & +4.5 & 14.36 & 0.02 & LCOGT-1m \\
58004.676 & +4.5 & 14.37 & 0.02 & LCOGT-1m \\
58005.080 & +4.9 & 14.30 & 0.06 & Konkoly \\
58005.128 & +4.9 & 14.29 & 0.02 & LCOGT-1m \\
58005.129 & +4.9 & 14.32 & 0.02 & LCOGT-1m \\
58010.765 & +10.6 & 14.26 & 0.01 & LCOGT-1m \\
58010.766 & +10.6 & 14.27 & 0.01 & LCOGT-1m \\
58011.600 & +11.4 & 14.34 & 0.08 & NOT \\
58011.781 & +11.6 & 14.28 & 0.01 & LCOGT-1m \\
58011.782 & +11.6 & 14.26 & 0.01 & LCOGT-1m \\
58013.745 & +13.5 & 14.28 & 0.01 & LCOGT-1m \\
58013.747 & +13.5 & 14.29 & 0.01 & LCOGT-1m \\
58014.700 & +14.5 & 14.41 & 0.02 & NOT \\
58015.003 & +14.8 & 14.28 & 0.01 & LCOGT-1m \\
58015.005 & +14.8 & 14.29 & 0.01 & LCOGT-1m \\
58015.748 & +15.5 & 14.33 & 0.01 & LCOGT-1m \\
58015.749 & +15.5 & 14.33 & 0.01 & LCOGT-1m \\
58016.570 & +16.4 & 14.37 & 0.01 & LCOGT-1m \\
58016.571 & +16.4 & 14.35 & 0.01 & LCOGT-1m \\
58017.550 & +17.3 & 14.45 & 0.01 & NOT \\
58019.300 & +19.1 & 14.40 & 0.04 & SLOTIS \\
58019.961 & +19.8 & 14.34 & 0.01 & LCOGT-1m \\
58019.963 & +19.8 & 14.35 & 0.01 & LCOGT-1m \\
58021.131 & +20.9 & 14.34 & 0.01 & LCOGT-1m \\
58021.132 & +20.9 & 14.35 & 0.01 & LCOGT-1m \\
58021.300 & +21.1 & 14.41 & 0.04 & SLOTIS \\
58022.300 & +22.1 & 14.42 & 0.04 & SLOTIS \\
58023.510 & +23.3 & 14.46 & 0.03 & NOT \\
58024.947 & +24.7 & 14.33 & 0.01 & LCOGT-1m \\
58024.948 & +24.7 & 14.32 & 0.01 & LCOGT-1m \\
58025.300 & +25.1 & 14.41 & 0.04 & SLOTIS \\
58028.500 & +28.3 & 14.40 & 0.07 & Liverpool \\
58029.174 & +29.0 & 14.38 & 0.01 & LCOGT-1m \\
58029.175 & +29.0 & 14.37 & 0.01 & LCOGT-1m \\
58032.300 & +32.1 & 14.45 & 0.06 & SLOTIS \\
58034.550 & +34.3 & 14.46 & 0.06 & Liverpool \\
58035.335 & +35.1 & 14.39 & 0.01 & LCOGT-1m \\
58035.336 & +35.1 & 14.39 & 0.01 & LCOGT-1m \\
58036.620 & +36.4 & 14.60 & 0.06 & NOT \\
58038.300 & +38.1 & 14.50 & 0.04 & SLOTIS \\
58039.342 & +39.1 & 14.40 & 0.01 & LCOGT-1m \\
58039.343 & +39.1 & 14.40 & 0.01 & LCOGT-1m \\
58041.300 & +41.1 & 14.52 & 0.04 & SLOTIS \\
58043.600 & +43.4 & 14.53 & 0.05 & Liverpool \\
58046.266 & +46.1 & 14.50 & 0.01 & LCOGT-1m \\
58046.268 & +46.1 & 14.50 & 0.01 & LCOGT-1m \\
58047.225 & +47.0 & 14.41 & 0.01 & LCOGT-1m \\
58047.227 & +47.0 & 14.42 & 0.01 & LCOGT-1m \\
58047.317 & +47.1 & 14.47 & 0.01 & LCOGT-1m \\
58047.319 & +47.1 & 14.46 & 0.01 & LCOGT-1m \\
58047.600 & +47.4 & 14.56 & 0.06 & NOT \\
58048.449 & +48.2 & 14.51 & 0.07 & Liverpool \\
58048.658 & +48.5 & 14.52 & 0.01 & LCOGT-1m \\
58048.660 & +48.5 & 14.53 & 0.01 & LCOGT-1m \\
58049.300 & +49.1 & 14.57 & 0.04 & SLOTIS \\
58051.560 & +51.4 & 14.63 & 0.04 & NOT \\
58052.866 & +52.7 & 14.50 & 0.01 & LCOGT-1m \\
58052.868 & +52.7 & 14.50 & 0.01 & LCOGT-1m \\
58053.200 & +53.0 & 14.61 & 0.04 & SLOTIS \\
58057.218 & +57.0 & 14.60 & 0.01 & LCOGT-1m \\
58057.220 & +57.0 & 14.59 & 0.01 & LCOGT-1m \\
58058.400 & +58.2 & 14.60 & 0.07 & Liverpool \\
58062.031 & +61.8 & 14.58 & 0.02 & LCOGT-1m \\
58062.033 & +61.8 & 14.60 & 0.02 & LCOGT-1m \\
58066.580 & +66.4 & 14.76 & 0.04 & NOT \\
58067.162 & +67.0 & 14.67 & 0.01 & LCOGT-1m \\
58067.164 & +67.0 & 14.69 & 0.01 & LCOGT-1m \\
58072.400 & +72.2 & 14.76 & 0.06 & Liverpool \\
58073.023 & +72.8 & 14.65 & 0.01 & LCOGT-1m \\
58073.025 & +72.8 & 14.62 & 0.01 & LCOGT-1m \\
58074.200 & +74.0 & 14.87 & 0.04 & SLOTIS \\
58077.200 & +77.0 & 14.93 & 0.04 & SLOTIS \\
58077.490 & +77.3 & 14.87 & 0.09 & Liverpool \\
58080.200 & +80.0 & 15.02 & 0.04 & SLOTIS \\
58080.554 & +80.4 & 14.90 & 0.01 & LCOGT-1m \\
58080.556 & +80.4 & 14.90 & 0.01 & LCOGT-1m \\
58083.200 & +83.0 & 15.11 & 0.04 & SLOTIS \\
58084.200 & +84.0 & 15.07 & 0.08 & Asiago-Schmidt \\
58087.078 & +86.9 & 15.13 & 0.01 & LCOGT-1m \\
58087.080 & +86.9 & 15.11 & 0.01 & LCOGT-1m \\
58089.815 & +89.6 & 15.32 & 0.02 & LCOGT-1m \\
58089.817 & +89.6 & 15.30 & 0.02 & LCOGT-1m \\
58090.800 & +90.6 & 15.40 & 0.07 & Asiago-Schmidt \\
58090.832 & +90.6 & 15.36 & 0.02 & LCOGT-1m \\
58090.834 & +90.6 & 15.35 & 0.02 & LCOGT-1m \\
58091.868 & +91.7 & 15.46 & 0.02 & LCOGT-1m \\
58091.870 & +91.7 & 15.39 & 0.02 & LCOGT-1m \\
58093.540 & +93.3 & 15.72 & 0.05 & NOT \\
58093.839 & +93.6 & 15.57 & 0.01 & LCOGT-1m \\
58093.841 & +93.6 & 15.55 & 0.01 & LCOGT-1m \\
58095.820 & +95.6 & 15.70 & 0.01 & LCOGT-1m \\
58095.822 & +95.6 & 15.68 & 0.01 & LCOGT-1m \\
58096.390 & +96.2 & 15.83 & 0.06 & Asiago-Schmidt \\
58096.806 & +96.6 & 15.74 & 0.01 & LCOGT-1m \\
58096.808 & +96.6 & 15.72 & 0.02 & LCOGT-1m \\
58097.155 & +97.0 & 15.85 & 0.01 & LCOGT-1m \\
58097.157 & +97.0 & 15.84 & 0.01 & LCOGT-1m \\
58099.230 & +99.0 & 16.10 & 0.07 & LCOGT-1m \\
58101.187 & +101.0 & 16.00 & 0.01 & LCOGT-1m \\
58101.189 & +101.0 & 16.02 & 0.01 & LCOGT-1m \\
58102.069 & +101.9 & 16.04 & 0.01 & LCOGT-1m \\
58102.071 & +101.9 & 16.04 & 0.01 & LCOGT-1m \\
58103.154 & +103.0 & 16.17 & 0.02 & LCOGT-1m \\
58103.156 & +103.0 & 16.18 & 0.02 & LCOGT-1m \\
58103.200 & +103.0 & 16.29 & 0.05 & SLOTIS \\
58104.183 & +104.0 & 16.17 & 0.01 & LCOGT-1m \\
58104.185 & +104.0 & 16.16 & 0.01 & LCOGT-1m \\
58104.400 & +104.2 & 16.26 & 0.08 & Liverpool \\
58105.280 & +105.1 & 16.27 & 0.06 & Asiago-Schmidt \\
58105.824 & +105.6 & 16.13 & 0.02 & LCOGT-1m \\
58105.827 & +105.6 & 16.16 & 0.02 & LCOGT-1m \\
58106.200 & +106.0 & 16.41 & 0.06 & SLOTIS \\
58109.340 & +109.1 & 16.29 & 0.07 & Liverpool \\
58109.340 & +109.1 & 16.29 & 0.07 & Asiago-Schmidt \\
58112.200 & +112.0 & 16.51 & 0.06 & SLOTIS \\
58113.863 & +113.7 & 16.35 & 0.02 & LCOGT-1m \\
58113.865 & +113.7 & 16.36 & 0.02 & LCOGT-1m \\
58114.430 & +114.2 & 16.47 & 0.06 & Liverpool \\
58121.867 & +121.7 & 16.50 & 0.02 & LCOGT-1m \\
58121.870 & +121.7 & 16.46 & 0.02 & LCOGT-1m \\
58123.100 & +122.9 & 16.69 & 0.08 & SLOTIS \\
58129.835 & +129.6 & 16.60 & 0.01 & LCOGT-1m \\
58129.838 & +129.6 & 16.60 & 0.02 & LCOGT-1m \\
58137.200 & +137.0 & 16.82 & 0.08 & SLOTIS \\
58137.380 & +137.2 & 16.88 & 0.04 & NOT \\
58139.085 & +138.9 & 16.69 & 0.01 & LCOGT-1m \\
58139.088 & +138.9 & 16.76 & 0.01 & LCOGT-1m \\
58146.200 & +146.0 & 17.10 & 0.09 & SLOTIS \\
58147.439 & +147.2 & 16.87 & 0.02 & LCOGT-1m \\
58147.442 & +147.2 & 16.89 & 0.02 & LCOGT-1m \\
58149.050 & +148.8 & 16.83 & 0.02 & LCOGT-1m \\
58156.425 & +156.2 & 17.01 & 0.02 & LCOGT-1m \\
58156.428 & +156.2 & 17.01 & 0.02 & LCOGT-1m \\
58163.340 & +163.1 & 17.21 & 0.05 & NOT \\
58164.027 & +163.8 & 17.10 & 0.02 & LCOGT-1m \\
58164.029 & +163.8 & 17.09 & 0.02 & LCOGT-1m \\
58172.021 & +171.8 & 17.14 & 0.03 & LCOGT-1m \\
58172.023 & +171.8 & 17.18 & 0.03 & LCOGT-1m \\
58173.029 & +172.8 & 17.04 & 0.03 & LCOGT-1m \\
58174.774 & +174.6 & 17.22 & 0.03 & LCOGT-1m \\
58174.776 & +174.6 & 17.18 & 0.03 & LCOGT-1m \\
58176.772 & +176.6 & 17.27 & 0.02 & LCOGT-1m \\
58176.775 & +176.6 & 17.23 & 0.02 & LCOGT-1m \\
\hline 
\multicolumn{5}{c}{$R$}\\
\hline 
58001.000 & +0.80 & 14.09 & 0.07 & Konkoly \\
58004.080 & +3.9 & 13.83 & 0.07 & Konkoly \\
58005.080 & +4.9 & 13.78 & 0.07 & Konkoly \\
58019.300 & +19.1 & 13.81 & 0.03 & SLOTIS \\
58021.300 & +21.1 & 13.81 & 0.02 & SLOTIS \\
58022.300 & +22.1 & 13.79 & 0.02 & SLOTIS \\
58025.300 & +25.1 & 13.78 & 0.02 & SLOTIS \\
58032.300 & +32.1 & 13.81 & 0.03 & SLOTIS \\
58038.300 & +38.1 & 13.82 & 0.03 & SLOTIS \\
58041.300 & +41.1 & 13.83 & 0.02 & SLOTIS \\
58049.300 & +49.1 & 13.86 & 0.02 & SLOTIS \\
58053.200 & +53.0 & 13.86 & 0.02 & SLOTIS \\
58074.200 & +74.0 & 13.96 & 0.02 & SLOTIS \\
58077.200 & +77.0 & 14.00 & 0.02 & SLOTIS \\
58080.200 & +80.0 & 14.06 & 0.03 & SLOTIS \\
58083.200 & +83.0 & 14.14 & 0.03 & SLOTIS \\
58103.200 & +103.0 & 15.11 & 0.05 & SLOTIS \\
58106.200 & +106.0 & 15.19 & 0.05 & SLOTIS \\
58112.200 & +112.0 & 15.27 & 0.06 & SLOTIS \\
58123.100 & +122.9 & 15.41 & 0.08 & SLOTIS \\
58137.200 & +137.0 & 15.54 & 0.05 & SLOTIS \\
58146.200 & +146.0 & 15.68 & 0.07 & SLOTIS \\
\hline 
\multicolumn{5}{c}{$I$}\\
\hline 
58001.000 & +0.80 & 14.13 & 0.06 & Konkoly \\
58004.080 & +3.9 & 13.69 & 0.07 & Konkoly \\
58005.080 & +4.9 & 13.62 & 0.07 & Konkoly \\
58019.300 & +19.1 & 13.67 & 0.02 & SLOTIS \\
58021.300 & +21.1 & 13.62 & 0.04 & SLOTIS \\
58022.300 & +22.1 & 13.64 & 0.02 & SLOTIS \\
58025.300 & +25.1 & 13.60 & 0.02 & SLOTIS \\
58032.300 & +32.1 & 13.58 & 0.03 & SLOTIS \\
58038.300 & +38.1 & 13.54 & 0.05 & SLOTIS \\
58041.300 & +41.1 & 13.58 & 0.02 & SLOTIS \\
58049.300 & +49.1 & 13.56 & 0.03 & SLOTIS \\
58053.200 & +53.0 & 13.57 & 0.02 & SLOTIS \\
58074.200 & +74.0 & 13.68 & 0.03 & SLOTIS \\
58077.200 & +77.0 & 13.71 & 0.05 & SLOTIS \\
58080.200 & +80.0 & 13.74 & 0.03 & SLOTIS \\
58083.200 & +83.0 & 13.81 & 0.03 & SLOTIS \\
58103.200 & +103.0 & 14.68 & 0.04 & SLOTIS \\
58106.200 & +106.0 & 14.77 & 0.05 & SLOTIS \\
58112.200 & +112.0 & 14.85 & 0.06 & SLOTIS \\
58123.100 & +122.9 & 15.00 & 0.06 & SLOTIS \\
58137.200 & +137.0 & 15.08 & 0.08 & SLOTIS \\
58146.200 & +146.0 & 15.22 & 0.07 & SLOTIS \\
\hline 
\multicolumn{5}{c}{$u$}\\
\hline 
58011.600 & +11.4 & 15.03 & 0.01 & NOT \\
58014.700 & +14.5 & 15.16 & 0.02 & NOT \\
58017.550 & +17.3 & 15.37 & 0.02 & NOT \\
58023.510 & +23.3 & 15.89 & 0.02 & NOT \\
58028.500 & +28.3 & 16.43 & 0.18 & Liverpool \\
58034.550 & +34.3 & 16.99 & 0.10 & Liverpool \\
58036.620 & +36.4 & 17.25 & 0.06 & NOT \\
58043.600 & +43.4 & 17.59 & 0.10 & Liverpool \\
58047.600 & +47.4 & 17.57 & 0.12 & NOT \\
58048.449 & +48.2 & 17.67 & 0.23 & Liverpool \\
58051.560 & +51.4 & 17.84 & 0.02 & NOT \\
\hline 
\multicolumn{5}{c}{$g$}\\
\hline 
58000.294 & +0.091 & 14.91 & 0.01 & LCOGT-1m \\
58000.297 & +0.094 & 14.92 & 0.01 & LCOGT-1m \\
58000.376 & +0.17 & 14.80 & 0.01 & LCOGT-1m \\
58000.379 & +0.18 & 14.78 & 0.01 & LCOGT-1m \\
58000.649 & +0.45 & 14.66 & 0.01 & LCOGT-1m \\
58000.651 & +0.45 & 14.67 & 0.01 & LCOGT-1m \\
58001.001 & +0.80 & 14.57 & 0.01 & LCOGT-1m \\
58001.004 & +0.80 & 14.53 & 0.01 & LCOGT-1m \\
58001.131 & +0.93 & 14.55 & 0.01 & LCOGT-1m \\
58001.134 & +0.93 & 14.53 & 0.01 & LCOGT-1m \\
58001.614 & +1.4 & 14.61 & 0.01 & LCOGT-1m \\
58001.617 & +1.4 & 14.56 & 0.01 & LCOGT-1m \\
58001.743 & +1.5 & 14.55 & 0.01 & LCOGT-1m \\
58001.746 & +1.5 & 14.57 & 0.01 & LCOGT-1m \\
58002.246 & +2.0 & 14.49 & 0.01 & LCOGT-1m \\
58002.249 & +2.0 & 14.50 & 0.01 & LCOGT-1m \\
58002.676 & +2.5 & 14.52 & 0.01 & LCOGT-1m \\
58002.679 & +2.5 & 14.54 & 0.01 & LCOGT-1m \\
58003.008 & +2.8 & 14.42 & 0.01 & LCOGT-1m \\
58003.010 & +2.8 & 14.43 & 0.01 & LCOGT-1m \\
58003.282 & +3.1 & 14.49 & 0.01 & LCOGT-1m \\
58003.285 & +3.1 & 14.48 & 0.01 & LCOGT-1m \\
58003.609 & +3.4 & 14.52 & 0.01 & LCOGT-1m \\
58003.611 & +3.4 & 14.59 & 0.01 & LCOGT-1m \\
58004.007 & +3.8 & 14.46 & 0.01 & LCOGT-1m \\
58004.009 & +3.8 & 14.43 & 0.01 & LCOGT-1m \\
58004.335 & +4.1 & 14.44 & 0.01 & LCOGT-1m \\
58004.337 & +4.1 & 14.39 & 0.01 & LCOGT-1m \\
58004.678 & +4.5 & 14.45 & 0.01 & LCOGT-1m \\
58004.680 & +4.5 & 14.50 & 0.01 & LCOGT-1m \\
58005.131 & +4.9 & 14.39 & 0.01 & LCOGT-1m \\
58005.133 & +4.9 & 14.38 & 0.01 & LCOGT-1m \\
58010.768 & +10.6 & 14.43 & 0.01 & LCOGT-1m \\
58010.771 & +10.6 & 14.43 & 0.01 & LCOGT-1m \\
58011.600 & +11.4 & 14.41 & 0.01 & NOT \\
58011.784 & +11.6 & 14.43 & 0.01 & LCOGT-1m \\
58011.786 & +11.6 & 14.44 & 0.01 & LCOGT-1m \\
58013.748 & +13.5 & 14.42 & 0.01 & LCOGT-1m \\
58013.751 & +13.5 & 14.42 & 0.01 & LCOGT-1m \\
58014.700 & +14.5 & 14.48 & 0.02 & NOT \\
58015.007 & +14.8 & 14.41 & 0.01 & LCOGT-1m \\
58015.009 & +14.8 & 14.41 & 0.01 & LCOGT-1m \\
58015.751 & +15.5 & 14.48 & 0.01 & LCOGT-1m \\
58015.753 & +15.6 & 14.48 & 0.01 & LCOGT-1m \\
58016.573 & +16.4 & 14.52 & 0.01 & LCOGT-1m \\
58016.576 & +16.4 & 14.51 & 0.01 & LCOGT-1m \\
58017.550 & +17.3 & 14.49 & 0.02 & NOT \\
58019.964 & +19.8 & 14.50 & 0.01 & LCOGT-1m \\
58019.967 & +19.8 & 14.50 & 0.01 & LCOGT-1m \\
58021.133 & +20.9 & 14.52 & 0.01 & LCOGT-1m \\
58021.135 & +20.9 & 14.52 & 0.01 & LCOGT-1m \\
58023.510 & +23.3 & 14.59 & 0.02 & NOT \\
58024.949 & +24.7 & 14.60 & 0.01 & LCOGT-1m \\
58024.951 & +24.7 & 14.60 & 0.01 & LCOGT-1m \\
58028.500 & +28.3 & 14.73 & 0.07 & Liverpool \\
58029.177 & +29.0 & 14.76 & 0.01 & LCOGT-1m \\
58029.178 & +29.0 & 14.73 & 0.01 & LCOGT-1m \\
58034.550 & +34.3 & 14.83 & 0.05 & Liverpool \\
58035.337 & +35.1 & 14.86 & 0.01 & LCOGT-1m \\
58035.339 & +35.1 & 14.80 & 0.01 & LCOGT-1m \\
58036.620 & +36.4 & 14.95 & 0.04 & NOT \\
58039.344 & +39.1 & 14.88 & 0.01 & LCOGT-1m \\
58039.346 & +39.1 & 14.88 & 0.01 & LCOGT-1m \\
58043.600 & +43.4 & 14.93 & 0.04 & Liverpool \\
58046.270 & +46.1 & 14.98 & 0.01 & LCOGT-1m \\
58046.273 & +46.1 & 14.97 & 0.01 & LCOGT-1m \\
58047.229 & +47.0 & 14.96 & 0.01 & LCOGT-1m \\
58047.232 & +47.0 & 14.96 & 0.01 & LCOGT-1m \\
58047.321 & +47.1 & 14.96 & 0.01 & LCOGT-1m \\
58047.324 & +47.1 & 14.97 & 0.01 & LCOGT-1m \\
58047.600 & +47.4 & 14.91 & 0.05 & NOT \\
58048.449 & +48.2 & 14.95 & 0.11 & Liverpool \\
58048.662 & +48.5 & 15.08 & 0.01 & LCOGT-1m \\
58048.665 & +48.5 & 15.07 & 0.01 & LCOGT-1m \\
58051.560 & +51.4 & 15.07 & 0.01 & NOT \\
58052.870 & +52.7 & 15.09 & 0.01 & LCOGT-1m \\
58052.873 & +52.7 & 15.09 & 0.01 & LCOGT-1m \\
58057.221 & +57.0 & 15.21 & 0.01 & LCOGT-1m \\
58057.224 & +57.0 & 15.19 & 0.01 & LCOGT-1m \\
58058.400 & +58.2 & 15.05 & 0.05 & Liverpool \\
58062.035 & +61.8 & 15.26 & 0.01 & LCOGT-1m \\
58062.038 & +61.8 & 15.25 & 0.01 & LCOGT-1m \\
58066.580 & +66.4 & 15.26 & 0.02 & NOT \\
58067.166 & +67.0 & 15.31 & 0.01 & LCOGT-1m \\
58067.168 & +67.0 & 15.31 & 0.01 & LCOGT-1m \\
58072.400 & +72.2 & 15.35 & 0.05 & Liverpool \\
58073.027 & +72.8 & 15.41 & 0.01 & LCOGT-1m \\
58073.030 & +72.8 & 15.40 & 0.01 & LCOGT-1m \\
58077.490 & +77.3 & 15.48 & 0.06 & Liverpool \\
58080.558 & +80.4 & 15.71 & 0.01 & LCOGT-1m \\
58080.561 & +80.4 & 15.71 & 0.01 & LCOGT-1m \\
58084.200 & +84.0 & 15.71 & 0.1 & Asiago-Schmidt \\
58087.082 & +86.9 & 15.92 & 0.01 & LCOGT-1m \\
58087.084 & +86.9 & 15.91 & 0.01 & LCOGT-1m \\
58089.819 & +89.6 & 16.27 & 0.01 & LCOGT-1m \\
58089.822 & +89.6 & 16.30 & 0.01 & LCOGT-1m \\
58090.800 & +90.6 & 16.12 & 0.07 & Asiago-Schmidt \\
58090.836 & +90.6 & 16.27 & 0.01 & LCOGT-1m \\
58090.839 & +90.6 & 16.25 & 0.01 & LCOGT-1m \\
58091.871 & +91.7 & 16.37 & 0.01 & LCOGT-1m \\
58091.874 & +91.7 & 16.36 & 0.01 & LCOGT-1m \\
58093.540 & +93.3 & 16.41 & 0.01 & NOT \\
58093.843 & +93.6 & 16.48 & 0.01 & LCOGT-1m \\
58093.846 & +93.6 & 16.48 & 0.01 & LCOGT-1m \\
58095.824 & +95.6 & 16.60 & 0.01 & LCOGT-1m \\
58095.827 & +95.6 & 16.59 & 0.01 & LCOGT-1m \\
58096.390 & +96.2 & 16.55 & 0.07 & Asiago-Schmidt \\
58096.810 & +96.6 & 16.63 & 0.01 & LCOGT-1m \\
58096.813 & +96.6 & 16.61 & 0.01 & LCOGT-1m \\
58097.159 & +97.0 & 16.76 & 0.01 & LCOGT-1m \\
58097.162 & +97.0 & 16.72 & 0.01 & LCOGT-1m \\
58099.232 & +99.0 & 16.59 & 0.01 & LCOGT-1m \\
58099.235 & +99.0 & 16.67 & 0.02 & LCOGT-1m \\
58101.191 & +101.0 & 16.90 & 0.01 & LCOGT-1m \\
58101.194 & +101.0 & 16.91 & 0.01 & LCOGT-1m \\
58102.073 & +101.9 & 16.87 & 0.01 & LCOGT-1m \\
58102.075 & +101.9 & 16.87 & 0.01 & LCOGT-1m \\
58103.158 & +103.0 & 17.06 & 0.01 & LCOGT-1m \\
58103.161 & +103.0 & 16.98 & 0.01 & LCOGT-1m \\
58104.187 & +104.0 & 17.11 & 0.01 & LCOGT-1m \\
58104.190 & +104.0 & 17.11 & 0.01 & LCOGT-1m \\
58104.400 & +104.2 & 16.90 & 0.05 & Liverpool \\
58105.280 & +105.1 & 16.97 & 0.06 & Asiago-Schmidt \\
58105.830 & +105.6 & 17.04 & 0.01 & LCOGT-1m \\
58105.834 & +105.6 & 17.00 & 0.01 & LCOGT-1m \\
58109.340 & +109.1 & 17.11 & 0.08 & Asiago-Schmidt \\
58109.340 & +109.1 & 17.11 & 0.08 & Liverpool \\
58113.868 & +113.7 & 17.24 & 0.01 & LCOGT-1m \\
58113.872 & +113.7 & 17.23 & 0.01 & LCOGT-1m \\
58114.430 & +114.2 & 17.06 & 0.06 & Liverpool \\
58121.873 & +121.7 & 17.34 & 0.01 & LCOGT-1m \\
58121.877 & +121.7 & 17.33 & 0.01 & LCOGT-1m \\
58129.841 & +129.6 & 17.40 & 0.01 & LCOGT-1m \\
58129.845 & +129.6 & 17.42 & 0.01 & LCOGT-1m \\
58137.380 & +137.2 & 17.44 & 0.01 & NOT \\
58139.091 & +138.9 & 17.51 & 0.01 & LCOGT-1m \\
58139.095 & +138.9 & 17.53 & 0.01 & LCOGT-1m \\
58149.056 & +148.9 & 17.72 & 0.02 & LCOGT-1m \\
58149.060 & +148.9 & 17.78 & 0.02 & LCOGT-1m \\
58156.431 & +156.2 & 17.70 & 0.01 & LCOGT-1m \\
58156.435 & +156.2 & 17.74 & 0.01 & LCOGT-1m \\
58163.340 & +163.1 & 17.72 & 0.01 & NOT \\
58164.035 & +163.8 & 17.83 & 0.01 & LCOGT-1m \\
58164.039 & +163.8 & 17.80 & 0.01 & LCOGT-1m \\
\hline 
\multicolumn{5}{c}{$r$}\\
\hline 
58000.203 & +0.0 & 15.11 & 0.02 & PROMPT5-DLT40 \\
58000.257 & +0.054 & 14.99 & 0.01 & PROMPT5-DLT40 \\
58000.300 & +0.097 & 14.99 & 0.01 & LCOGT-1m \\
58000.301 & +0.098 & 14.99 & 0.01 & LCOGT-1m \\
58000.382 & +0.18 & 14.94 & 0.01 & LCOGT-1m \\
58000.383 & +0.18 & 14.95 & 0.01 & LCOGT-1m \\
58000.654 & +0.45 & 14.74 & 0.01 & LCOGT-1m \\
58000.656 & +0.45 & 14.70 & 0.01 & LCOGT-1m \\
58001.007 & +0.80 & 14.62 & 0.01 & LCOGT-1m \\
58001.009 & +0.81 & 14.60 & 0.01 & LCOGT-1m \\
58001.137 & +0.93 & 14.59 & 0.01 & LCOGT-1m \\
58001.138 & +0.94 & 14.58 & 0.01 & LCOGT-1m \\
58001.227 & +1.0 & 14.47 & 0.01 & PROMPT5-DLT40 \\
58001.620 & +1.4 & 14.65 & 0.02 & LCOGT-1m \\
58001.621 & +1.4 & 14.65 & 0.01 & LCOGT-1m \\
58001.748 & +1.5 & 14.58 & 0.01 & LCOGT-1m \\
58001.750 & +1.5 & 14.58 & 0.01 & LCOGT-1m \\
58002.251 & +2.0 & 14.49 & 0.01 & LCOGT-1m \\
58002.253 & +2.1 & 14.56 & 0.01 & LCOGT-1m \\
58002.682 & +2.5 & 14.47 & 0.01 & LCOGT-1m \\
58002.683 & +2.5 & 14.46 & 0.01 & LCOGT-1m \\
58003.013 & +2.8 & 14.38 & 0.01 & LCOGT-1m \\
58003.015 & +2.8 & 14.36 & 0.01 & LCOGT-1m \\
58003.157 & +3.0 & 14.27 & 0.01 & PROMPT5-DLT40 \\
58003.288 & +3.1 & 14.30 & 0.01 & LCOGT-1m \\
58003.289 & +3.1 & 14.30 & 0.01 & LCOGT-1m \\
58003.614 & +3.4 & 14.37 & 0.01 & LCOGT-1m \\
58003.615 & +3.4 & 14.38 & 0.01 & LCOGT-1m \\
58004.012 & +3.8 & 14.28 & 0.01 & LCOGT-1m \\
58004.014 & +3.8 & 14.28 & 0.01 & LCOGT-1m \\
58004.215 & +4.0 & 14.19 & 0.01 & PROMPT5-DLT40 \\
58004.340 & +4.1 & 14.37 & 0.01 & LCOGT-1m \\
58004.342 & +4.1 & 14.39 & 0.01 & LCOGT-1m \\
58004.683 & +4.5 & 14.29 & 0.01 & LCOGT-1m \\
58004.684 & +4.5 & 14.24 & 0.01 & LCOGT-1m \\
58005.136 & +4.9 & 14.22 & 0.01 & LCOGT-1m \\
58005.138 & +4.9 & 14.23 & 0.01 & LCOGT-1m \\
58010.773 & +10.6 & 14.09 & 0.01 & LCOGT-1m \\
58010.775 & +10.6 & 14.10 & 0.01 & LCOGT-1m \\
58011.133 & +10.9 & 14.06 & 0.01 & PROMPT5-DLT40 \\
58011.600 & +11.4 & 14.14 & 0.05 & NOT \\
58011.789 & +11.6 & 14.16 & 0.01 & LCOGT-1m \\
58011.791 & +11.6 & 14.17 & 0.01 & LCOGT-1m \\
58012.130 & +11.9 & 14.05 & 0.01 & PROMPT5-DLT40 \\
58013.754 & +13.6 & 14.11 & 0.01 & LCOGT-1m \\
58013.755 & +13.6 & 14.11 & 0.01 & LCOGT-1m \\
58014.127 & +13.9 & 14.02 & 0.01 & PROMPT5-DLT40 \\
58014.700 & +14.5 & 14.16 & 0.05 & NOT \\
58015.012 & +14.8 & 14.09 & 0.01 & LCOGT-1m \\
58015.013 & +14.8 & 14.07 & 0.01 & LCOGT-1m \\
58015.158 & +15.0 & 14.04 & 0.01 & PROMPT5-DLT40 \\
58015.756 & +15.6 & 14.16 & 0.01 & LCOGT-1m \\
58015.758 & +15.6 & 14.16 & 0.01 & LCOGT-1m \\
58016.578 & +16.4 & 14.14 & 0.01 & LCOGT-1m \\
58016.580 & +16.4 & 14.15 & 0.01 & LCOGT-1m \\
58017.117 & +16.9 & 14.06 & 0.01 & PROMPT5-DLT40 \\
58017.550 & +17.3 & 14.18 & 0.04 & NOT \\
58018.114 & +17.9 & 14.12 & 0.01 & PROMPT5-DLT40 \\
58019.114 & +18.9 & 14.10 & 0.01 & PROMPT5-DLT40 \\
58019.970 & +19.8 & 14.11 & 0.01 & LCOGT-1m \\
58019.971 & +19.8 & 14.09 & 0.01 & LCOGT-1m \\
58021.106 & +20.9 & 14.11 & 0.02 & PROMPT5-DLT40 \\
58021.137 & +20.9 & 14.08 & 0.01 & LCOGT-1m \\
58021.138 & +20.9 & 14.08 & 0.01 & LCOGT-1m \\
58022.149 & +21.9 & 14.12 & 0.02 & PROMPT5-DLT40 \\
58024.953 & +24.7 & 14.06 & 0.01 & LCOGT-1m \\
58024.954 & +24.8 & 14.03 & 0.01 & LCOGT-1m \\
58028.087 & +27.9 & 13.96 & 0.02 & PROMPT5-DLT40 \\
58028.500 & +28.3 & 14.11 & 0.05 & Liverpool \\
58029.084 & +28.9 & 14.11 & 0.01 & PROMPT5-DLT40 \\
58029.180 & +29.0 & 14.10 & 0.01 & LCOGT-1m \\
58029.181 & +29.0 & 14.08 & 0.01 & LCOGT-1m \\
58030.082 & +29.9 & 14.05 & 0.03 & PROMPT5-DLT40 \\
58032.076 & +31.9 & 14.15 & 0.03 & PROMPT5-DLT40 \\
58034.071 & +33.9 & 14.17 & 0.01 & PROMPT5-DLT40 \\
58034.550 & +34.3 & 14.14 & 0.05 & Liverpool \\
58035.068 & +34.9 & 14.14 & 0.01 & PROMPT5-DLT40 \\
58035.341 & +35.1 & 14.16 & 0.01 & LCOGT-1m \\
58035.342 & +35.1 & 14.15 & 0.01 & LCOGT-1m \\
58036.070 & +35.9 & 14.19 & 0.01 & PROMPT5-DLT40 \\
58036.620 & +36.4 & 14.20 & 0.03 & NOT \\
58037.063 & +36.9 & 14.16 & 0.01 & PROMPT5-DLT40 \\
58038.066 & +37.9 & 14.16 & 0.01 & PROMPT5-DLT40 \\
58039.060 & +38.9 & 14.19 & 0.01 & PROMPT5-DLT40 \\
58039.348 & +39.1 & 14.11 & 0.01 & LCOGT-1m \\
58039.349 & +39.1 & 14.14 & 0.01 & LCOGT-1m \\
58040.054 & +39.9 & 14.15 & 0.01 & PROMPT5-DLT40 \\
58041.051 & +40.8 & 14.17 & 0.01 & PROMPT5-DLT40 \\
58043.046 & +42.8 & 14.22 & 0.01 & PROMPT5-DLT40 \\
58043.600 & +43.4 & 14.17 & 0.05 & Liverpool \\
58044.224 & +44.0 & 14.21 & 0.01 & PROMPT5-DLT40 \\
58045.041 & +44.8 & 14.15 & 0.01 & PROMPT5-DLT40 \\
58046.038 & +45.8 & 14.21 & 0.01 & PROMPT5-DLT40 \\
58046.276 & +46.1 & 14.16 & 0.01 & LCOGT-1m \\
58046.277 & +46.1 & 14.16 & 0.01 & LCOGT-1m \\
58047.035 & +46.8 & 14.18 & 0.01 & PROMPT5-DLT40 \\
58047.234 & +47.0 & 14.09 & 0.01 & LCOGT-1m \\
58047.327 & +47.1 & 14.12 & 0.01 & LCOGT-1m \\
58047.328 & +47.1 & 14.12 & 0.01 & LCOGT-1m \\
58047.600 & +47.4 & 14.21 & 0.09 & NOT \\
58048.032 & +47.8 & 14.21 & 0.01 & PROMPT5-DLT40 \\
58048.449 & +48.2 & 14.16 & 0.07 & Liverpool \\
58048.667 & +48.5 & 14.21 & 0.01 & LCOGT-1m \\
58048.669 & +48.5 & 14.21 & 0.01 & LCOGT-1m \\
58050.027 & +49.8 & 14.22 & 0.01 & PROMPT5-DLT40 \\
58051.025 & +50.8 & 14.19 & 0.01 & PROMPT5-DLT40 \\
58051.560 & +51.4 & 14.24 & 0.05 & NOT \\
58052.021 & +51.8 & 14.20 & 0.01 & PROMPT5-DLT40 \\
58052.876 & +52.7 & 14.18 & 0.01 & LCOGT-1m \\
58052.877 & +52.7 & 14.17 & 0.01 & LCOGT-1m \\
58053.018 & +52.8 & 14.23 & 0.01 & PROMPT5-DLT40 \\
58057.008 & +56.8 & 14.22 & 0.01 & PROMPT5-DLT40 \\
58057.227 & +57.0 & 14.24 & 0.01 & LCOGT-1m \\
58057.229 & +57.0 & 14.24 & 0.01 & LCOGT-1m \\
58058.005 & +57.8 & 14.21 & 0.01 & PROMPT5-DLT40 \\
58058.400 & +58.2 & 14.19 & 0.05 & Liverpool \\
58062.041 & +61.8 & 14.20 & 0.01 & LCOGT-1m \\
58062.042 & +61.8 & 14.22 & 0.01 & LCOGT-1m \\
58062.082 & +61.9 & 14.23 & 0.02 & PROMPT5-DLT40 \\
58063.004 & +62.8 & 14.24 & 0.01 & PROMPT5-DLT40 \\
58065.006 & +64.8 & 14.29 & 0.01 & PROMPT5-DLT40 \\
58066.006 & +65.8 & 14.30 & 0.01 & PROMPT5-DLT40 \\
58066.580 & +66.4 & 14.27 & 0.07 & NOT \\
58067.007 & +66.8 & 14.25 & 0.01 & PROMPT5-DLT40 \\
58067.171 & +67.0 & 14.29 & 0.01 & LCOGT-1m \\
58067.173 & +67.0 & 14.28 & 0.01 & LCOGT-1m \\
58068.008 & +67.8 & 14.27 & 0.01 & PROMPT5-DLT40 \\
58069.008 & +68.8 & 14.33 & 0.02 & PROMPT5-DLT40 \\
58070.009 & +69.8 & 14.25 & 0.02 & PROMPT5-DLT40 \\
58071.010 & +70.8 & 14.26 & 0.01 & PROMPT5-DLT40 \\
58072.010 & +71.8 & 14.29 & 0.01 & PROMPT5-DLT40 \\
58072.400 & +72.2 & 14.28 & 0.03 & Liverpool \\
58073.032 & +72.8 & 14.23 & 0.01 & LCOGT-1m \\
58073.034 & +72.8 & 14.24 & 0.01 & LCOGT-1m \\
58077.490 & +77.3 & 14.36 & 0.05 & Liverpool \\
58078.015 & +77.8 & 14.49 & 0.01 & PROMPT5-DLT40 \\
58079.015 & +78.8 & 14.43 & 0.01 & PROMPT5-DLT40 \\
58080.016 & +79.8 & 14.46 & 0.02 & PROMPT5-DLT40 \\
58080.564 & +80.4 & 14.41 & 0.01 & LCOGT-1m \\
58080.565 & +80.4 & 14.41 & 0.01 & LCOGT-1m \\
58081.017 & +80.8 & 14.48 & 0.01 & PROMPT5-DLT40 \\
58082.017 & +81.8 & 14.55 & 0.01 & PROMPT5-DLT40 \\
58083.018 & +82.8 & 14.56 & 0.01 & PROMPT5-DLT40 \\
58084.019 & +83.8 & 14.55 & 0.01 & PROMPT5-DLT40 \\
58084.200 & +84.0 & 14.59 & 0.08 & Asiago-Schmidt \\
58085.019 & +84.8 & 14.57 & 0.02 & PROMPT5-DLT40 \\
58087.021 & +86.8 & 14.62 & 0.01 & PROMPT5-DLT40 \\
58087.087 & +86.9 & 14.55 & 0.01 & LCOGT-1m \\
58087.089 & +86.9 & 14.56 & 0.01 & LCOGT-1m \\
58089.210 & +89.0 & 14.70 & 0.02 & PROMPT5-DLT40 \\
58089.825 & +89.6 & 14.75 & 0.01 & LCOGT-1m \\
58089.827 & +89.6 & 14.71 & 0.01 & LCOGT-1m \\
58090.030 & +89.8 & 14.81 & 0.01 & PROMPT5-DLT40 \\
58090.800 & +90.6 & 14.80 & 0.06 & Asiago-Schmidt \\
58090.842 & +90.6 & 14.74 & 0.01 & LCOGT-1m \\
58090.844 & +90.6 & 14.72 & 0.01 & LCOGT-1m \\
58091.877 & +91.7 & 14.82 & 0.01 & LCOGT-1m \\
58091.879 & +91.7 & 14.84 & 0.01 & LCOGT-1m \\
58092.191 & +92.0 & 14.90 & 0.01 & PROMPT5-DLT40 \\
58093.028 & +92.8 & 14.99 & 0.01 & PROMPT5-DLT40 \\
58093.540 & +93.3 & 15.04 & 0.05 & NOT \\
58093.849 & +93.6 & 14.93 & 0.01 & LCOGT-1m \\
58093.851 & +93.6 & 14.94 & 0.01 & LCOGT-1m \\
58095.026 & +94.8 & 15.04 & 0.02 & PROMPT5-DLT40 \\
58095.830 & +95.6 & 15.04 & 0.01 & LCOGT-1m \\
58095.832 & +95.6 & 15.01 & 0.01 & LCOGT-1m \\
58096.026 & +95.8 & 15.15 & 0.03 & PROMPT5-DLT40 \\
58096.390 & +96.2 & 15.18 & 0.06 & Asiago-Schmidt \\
58096.816 & +96.6 & 15.06 & 0.01 & LCOGT-1m \\
58096.817 & +96.6 & 15.07 & 0.01 & LCOGT-1m \\
58097.027 & +96.8 & 15.16 & 0.03 & PROMPT5-DLT40 \\
58097.165 & +97.0 & 15.17 & 0.01 & LCOGT-1m \\
58097.167 & +97.0 & 15.19 & 0.01 & LCOGT-1m \\
58098.027 & +97.8 & 15.25 & 0.02 & PROMPT5-DLT40 \\
58099.238 & +99.0 & 15.35 & 0.01 & LCOGT-1m \\
58100.029 & +99.8 & 15.35 & 0.01 & PROMPT5-DLT40 \\
58101.029 & +100.8 & 15.33 & 0.04 & PROMPT5-DLT40 \\
58101.197 & +101.0 & 15.30 & 0.01 & LCOGT-1m \\
58101.198 & +101.0 & 15.31 & 0.01 & LCOGT-1m \\
58102.029 & +101.8 & 15.37 & 0.04 & PROMPT5-DLT40 \\
58102.078 & +101.9 & 15.32 & 0.01 & LCOGT-1m \\
58102.080 & +101.9 & 15.31 & 0.01 & LCOGT-1m \\
58103.030 & +102.8 & 15.45 & 0.03 & PROMPT5-DLT40 \\
58103.163 & +103.0 & 15.46 & 0.01 & LCOGT-1m \\
58103.165 & +103.0 & 15.46 & 0.01 & LCOGT-1m \\
58104.031 & +103.8 & 15.53 & 0.03 & PROMPT5-DLT40 \\
58104.193 & +104.0 & 15.51 & 0.01 & LCOGT-1m \\
58104.195 & +104.0 & 15.51 & 0.01 & LCOGT-1m \\
58104.400 & +104.2 & 15.45 & 0.05 & Liverpool \\
58105.031 & +104.8 & 15.44 & 0.05 & PROMPT5-DLT40 \\
58105.280 & +105.1 & 15.51 & 0.06 & Asiago-Schmidt \\
58105.838 & +105.6 & 15.42 & 0.01 & LCOGT-1m \\
58105.841 & +105.6 & 15.37 & 0.01 & LCOGT-1m \\
58106.031 & +105.8 & 15.58 & 0.07 & PROMPT5-DLT40 \\
58107.032 & +106.8 & 15.52 & 0.04 & PROMPT5-DLT40 \\
58108.032 & +107.8 & 15.60 & 0.02 & PROMPT5-DLT40 \\
58109.032 & +108.8 & 15.49 & 0.04 & PROMPT5-DLT40 \\
58109.340 & +109.1 & 15.64 & 0.07 & Liverpool \\
58109.340 & +109.1 & 15.64 & 0.07 & Asiago-Schmidt \\
58110.033 & +109.8 & 15.62 & 0.02 & PROMPT5-DLT40 \\
58111.033 & +110.8 & 15.60 & 0.02 & PROMPT5-DLT40 \\
58111.516 & +111.3 & 15.56 & 0.03 & PROMPTMO-DLT40 \\
58112.033 & +111.8 & 15.66 & 0.03 & PROMPT5-DLT40 \\
58112.546 & +112.3 & 15.62 & 0.02 & PROMPTMO-DLT40 \\
58113.034 & +112.8 & 15.76 & 0.04 & PROMPT5-DLT40 \\
58113.541 & +113.3 & 15.67 & 0.01 & PROMPTMO-DLT40 \\
58113.876 & +113.7 & 15.55 & 0.01 & LCOGT-1m \\
58113.879 & +113.7 & 15.55 & 0.01 & LCOGT-1m \\
58114.034 & +113.8 & 15.64 & 0.03 & PROMPT5-DLT40 \\
58114.430 & +114.2 & 15.59 & 0.03 & Liverpool \\
58115.034 & +114.8 & 15.73 & 0.05 & PROMPT5-DLT40 \\
58115.516 & +115.3 & 15.57 & 0.05 & PROMPTMO-DLT40 \\
58116.519 & +116.3 & 15.71 & 0.02 & PROMPTMO-DLT40 \\
58117.034 & +116.8 & 15.80 & 0.03 & PROMPT5-DLT40 \\
58117.519 & +117.3 & 15.57 & 0.02 & PROMPTMO-DLT40 \\
58118.034 & +117.8 & 15.90 & 0.03 & PROMPT5-DLT40 \\
58118.519 & +118.3 & 15.72 & 0.02 & PROMPTMO-DLT40 \\
58119.038 & +118.8 & 15.77 & 0.02 & PROMPT5-DLT40 \\
58119.519 & +119.3 & 15.90 & 0.02 & PROMPTMO-DLT40 \\
58120.038 & +119.8 & 15.75 & 0.05 & PROMPT5-DLT40 \\
58121.038 & +120.8 & 15.76 & 0.03 & PROMPT5-DLT40 \\
58121.881 & +121.7 & 15.65 & 0.01 & LCOGT-1m \\
58121.884 & +121.7 & 15.64 & 0.01 & LCOGT-1m \\
58122.038 & +121.8 & 15.83 & 0.03 & PROMPT5-DLT40 \\
58122.519 & +122.3 & 15.76 & 0.02 & PROMPTMO-DLT40 \\
58123.519 & +123.3 & 15.81 & 0.02 & PROMPTMO-DLT40 \\
58124.520 & +124.3 & 15.80 & 0.03 & PROMPTMO-DLT40 \\
58125.038 & +124.8 & 15.76 & 0.18 & PROMPT5-DLT40 \\
58125.519 & +125.3 & 15.59 & 0.10 & PROMPTMO-DLT40 \\
58126.082 & +125.9 & 15.74 & 0.03 & PROMPT5-DLT40 \\
58127.038 & +126.8 & 15.83 & 0.03 & PROMPT5-DLT40 \\
58128.038 & +127.8 & 15.85 & 0.03 & PROMPT5-DLT40 \\
58128.519 & +128.3 & 15.67 & 0.03 & PROMPTMO-DLT40 \\
58129.039 & +128.8 & 15.85 & 0.04 & PROMPT5-DLT40 \\
58129.522 & +129.3 & 15.83 & 0.02 & PROMPTMO-DLT40 \\
58129.849 & +129.6 & 15.71 & 0.01 & LCOGT-1m \\
58129.852 & +129.6 & 15.73 & 0.01 & LCOGT-1m \\
58130.044 & +129.8 & 15.70 & 0.04 & PROMPT5-DLT40 \\
58130.519 & +130.3 & 15.83 & 0.03 & PROMPTMO-DLT40 \\
58131.520 & +131.3 & 15.87 & 0.02 & PROMPTMO-DLT40 \\
58133.037 & +132.8 & 15.89 & 0.02 & PROMPT5-DLT40 \\
58134.036 & +133.8 & 15.93 & 0.02 & PROMPT5-DLT40 \\
58135.037 & +134.8 & 16.00 & 0.03 & PROMPT5-DLT40 \\
58136.036 & +135.8 & 15.98 & 0.04 & PROMPT5-DLT40 \\
58137.036 & +136.8 & 15.92 & 0.04 & PROMPT5-DLT40 \\
58137.380 & +137.2 & 15.95 & 0.06 & NOT \\
58137.517 & +137.3 & 15.86 & 0.04 & PROMPTMO-DLT40 \\
58138.036 & +137.8 & 15.92 & 0.04 & PROMPT5-DLT40 \\
58139.099 & +138.9 & 15.83 & 0.01 & LCOGT-1m \\
58139.101 & +138.9 & 15.84 & 0.01 & LCOGT-1m \\
58139.608 & +139.4 & 16.00 & 0.02 & PROMPTMO-DLT40 \\
58140.034 & +139.8 & 16.07 & 0.03 & PROMPT5-DLT40 \\
58140.516 & +140.3 & 15.91 & 0.04 & PROMPTMO-DLT40 \\
58141.558 & +141.4 & 15.95 & 0.03 & PROMPTMO-DLT40 \\
58144.096 & +143.9 & 15.99 & 0.08 & PROMPT5-DLT40 \\
58145.033 & +144.8 & 15.78 & 0.07 & PROMPT5-DLT40 \\
58145.514 & +145.3 & 16.05 & 0.04 & PROMPTMO-DLT40 \\
58146.032 & +145.8 & 15.85 & 0.09 & PROMPT5-DLT40 \\
58146.514 & +146.3 & 16.09 & 0.02 & PROMPTMO-DLT40 \\
58147.032 & +146.8 & 16.02 & 0.09 & PROMPT5-DLT40 \\
58148.031 & +147.8 & 16.10 & 0.02 & PROMPT5-DLT40 \\
58148.514 & +148.3 & 15.96 & 0.02 & PROMPTMO-DLT40 \\
58149.030 & +148.8 & 16.07 & 0.02 & PROMPT5-DLT40 \\
58149.064 & +148.9 & 15.88 & 0.01 & LCOGT-1m \\
58149.067 & +148.9 & 15.94 & 0.01 & LCOGT-1m \\
58149.511 & +149.3 & 16.02 & 0.02 & PROMPTMO-DLT40 \\
58150.030 & +149.8 & 16.18 & 0.02 & PROMPT5-DLT40 \\
58151.029 & +150.8 & 16.14 & 0.02 & PROMPT5-DLT40 \\
58151.510 & +151.3 & 16.05 & 0.02 & PROMPTMO-DLT40 \\
58152.029 & +151.8 & 16.25 & 0.02 & PROMPT5-DLT40 \\
58153.028 & +152.8 & 16.17 & 0.02 & PROMPT5-DLT40 \\
58153.509 & +153.3 & 16.15 & 0.03 & PROMPTMO-DLT40 \\
58156.439 & +156.2 & 16.00 & 0.01 & LCOGT-1m \\
58156.442 & +156.2 & 16.02 & 0.01 & LCOGT-1m \\
58157.024 & +156.8 & 16.20 & 0.05 & PROMPT5-DLT40 \\
58158.025 & +157.8 & 16.26 & 0.02 & PROMPT5-DLT40 \\
58163.340 & +163.1 & 16.25 & 0.06 & NOT \\
58164.043 & +163.8 & 16.14 & 0.01 & LCOGT-1m \\
58164.046 & +163.8 & 16.15 & 0.01 & LCOGT-1m \\
\hline 
\multicolumn{5}{c}{$i$}\\
\hline 
58000.303 & +0.10 & 15.06 & 0.01 & LCOGT-1m \\
58000.305 & +0.10 & 15.05 & 0.01 & LCOGT-1m \\
58000.385 & +0.18 & 14.96 & 0.01 & LCOGT-1m \\
58000.387 & +0.18 & 14.97 & 0.01 & LCOGT-1m \\
58000.658 & +0.46 & 14.76 & 0.01 & LCOGT-1m \\
58000.660 & +0.46 & 14.74 & 0.01 & LCOGT-1m \\
58001.011 & +0.81 & 14.63 & 0.01 & LCOGT-1m \\
58001.013 & +0.81 & 14.62 & 0.01 & LCOGT-1m \\
58001.140 & +0.94 & 14.61 & 0.01 & LCOGT-1m \\
58001.142 & +0.94 & 14.60 & 0.01 & LCOGT-1m \\
58001.623 & +1.4 & 14.61 & 0.01 & LCOGT-1m \\
58001.624 & +1.4 & 14.61 & 0.01 & LCOGT-1m \\
58001.751 & +1.5 & 14.54 & 0.01 & LCOGT-1m \\
58001.753 & +1.6 & 14.56 & 0.01 & LCOGT-1m \\
58002.255 & +2.1 & 14.48 & 0.01 & LCOGT-1m \\
58002.256 & +2.1 & 14.47 & 0.01 & LCOGT-1m \\
58002.685 & +2.5 & 14.42 & 0.01 & LCOGT-1m \\
58002.686 & +2.5 & 14.42 & 0.01 & LCOGT-1m \\
58003.016 & +2.8 & 14.34 & 0.01 & LCOGT-1m \\
58003.018 & +2.8 & 14.33 & 0.01 & LCOGT-1m \\
58003.291 & +3.1 & 14.39 & 0.01 & LCOGT-1m \\
58003.292 & +3.1 & 14.39 & 0.01 & LCOGT-1m \\
58003.617 & +3.4 & 14.32 & 0.01 & LCOGT-1m \\
58003.619 & +3.4 & 14.30 & 0.01 & LCOGT-1m \\
58004.015 & +3.8 & 14.23 & 0.01 & LCOGT-1m \\
58004.017 & +3.8 & 14.23 & 0.01 & LCOGT-1m \\
58004.344 & +4.1 & 14.24 & 0.01 & LCOGT-1m \\
58004.345 & +4.1 & 14.27 & 0.01 & LCOGT-1m \\
58004.686 & +4.5 & 14.19 & 0.01 & LCOGT-1m \\
58004.688 & +4.5 & 14.21 & 0.01 & LCOGT-1m \\
58005.140 & +4.9 & 14.16 & 0.01 & LCOGT-1m \\
58005.141 & +4.9 & 14.17 & 0.01 & LCOGT-1m \\
58010.777 & +10.6 & 14.04 & 0.01 & LCOGT-1m \\
58010.778 & +10.6 & 14.04 & 0.01 & LCOGT-1m \\
58011.600 & +11.4 & 14.03 & 0.04 & NOT \\
58011.792 & +11.6 & 14.07 & 0.01 & LCOGT-1m \\
58011.794 & +11.6 & 14.08 & 0.01 & LCOGT-1m \\
58013.757 & +13.6 & 14.07 & 0.01 & LCOGT-1m \\
58013.759 & +13.6 & 14.08 & 0.01 & LCOGT-1m \\
58014.700 & +14.5 & 14.14 & 0.03 & NOT \\
58015.015 & +14.8 & 14.04 & 0.01 & LCOGT-1m \\
58015.017 & +14.8 & 14.05 & 0.01 & LCOGT-1m \\
58015.759 & +15.6 & 14.13 & 0.01 & LCOGT-1m \\
58015.761 & +15.6 & 14.12 & 0.01 & LCOGT-1m \\
58016.582 & +16.4 & 14.15 & 0.01 & LCOGT-1m \\
58016.583 & +16.4 & 14.15 & 0.01 & LCOGT-1m \\
58017.550 & +17.3 & 14.12 & 0.02 & NOT \\
58019.973 & +19.8 & 14.13 & 0.01 & LCOGT-1m \\
58019.974 & +19.8 & 14.13 & 0.01 & LCOGT-1m \\
58021.139 & +20.9 & 14.08 & 0.01 & LCOGT-1m \\
58021.140 & +20.9 & 14.09 & 0.01 & LCOGT-1m \\
58023.510 & +23.3 & 14.05 & 0.05 & NOT \\
58024.955 & +24.8 & 14.05 & 0.01 & LCOGT-1m \\
58024.956 & +24.8 & 14.05 & 0.01 & LCOGT-1m \\
58028.500 & +28.3 & 14.11 & 0.06 & Liverpool \\
58029.183 & +29.0 & 14.08 & 0.01 & LCOGT-1m \\
58029.184 & +29.0 & 14.09 & 0.01 & LCOGT-1m \\
58034.550 & +34.3 & 14.09 & 0.06 & Liverpool \\
58035.343 & +35.1 & 14.02 & 0.01 & LCOGT-1m \\
58035.344 & +35.1 & 14.12 & 0.01 & LCOGT-1m \\
58036.620 & +36.4 & 14.13 & 0.03 & NOT \\
58039.350 & +39.1 & 14.07 & 0.01 & LCOGT-1m \\
58039.351 & +39.1 & 14.08 & 0.01 & LCOGT-1m \\
58043.600 & +43.4 & 14.08 & 0.05 & Liverpool \\
58046.280 & +46.1 & 14.10 & 0.01 & LCOGT-1m \\
58046.282 & +46.1 & 14.07 & 0.01 & LCOGT-1m \\
58047.263 & +47.1 & 14.00 & 0.01 & LCOGT-1m \\
58047.265 & +47.1 & 13.99 & 0.01 & LCOGT-1m \\
58047.331 & +47.1 & 14.04 & 0.01 & LCOGT-1m \\
58047.332 & +47.1 & 14.04 & 0.01 & LCOGT-1m \\
58047.600 & +47.4 & 14.09 & 0.03 & NOT \\
58048.449 & +48.2 & 14.05 & 0.1 & Liverpool \\
58048.672 & +48.5 & 14.08 & 0.01 & LCOGT-1m \\
58048.673 & +48.5 & 14.09 & 0.01 & LCOGT-1m \\
58051.560 & +51.4 & 14.12 & 0.03 & NOT \\
58052.879 & +52.7 & 14.10 & 0.01 & LCOGT-1m \\
58052.881 & +52.7 & 14.11 & 0.01 & LCOGT-1m \\
58057.231 & +57.0 & 14.13 & 0.01 & LCOGT-1m \\
58057.233 & +57.0 & 14.12 & 0.01 & LCOGT-1m \\
58058.400 & +58.2 & 14.10 & 0.05 & Liverpool \\
58062.044 & +61.8 & 14.07 & 0.01 & LCOGT-1m \\
58062.046 & +61.8 & 14.08 & 0.01 & LCOGT-1m \\
58066.580 & +66.4 & 14.14 & 0.02 & NOT \\
58067.175 & +67.0 & 14.13 & 0.01 & LCOGT-1m \\
58067.177 & +67.0 & 14.16 & 0.01 & LCOGT-1m \\
58072.400 & +72.2 & 14.12 & 0.02 & Liverpool \\
58073.036 & +72.8 & 14.13 & 0.01 & LCOGT-1m \\
58073.038 & +72.8 & 14.13 & 0.01 & LCOGT-1m \\
58077.490 & +77.3 & 14.16 & 0.02 & Liverpool \\
58080.567 & +80.4 & 14.16 & 0.01 & LCOGT-1m \\
58080.569 & +80.4 & 14.21 & 0.01 & LCOGT-1m \\
58084.200 & +84.0 & 14.31 & 0.09 & Asiago-Schmidt \\
58087.091 & +86.9 & 14.36 & 0.01 & LCOGT-1m \\
58087.093 & +86.9 & 14.37 & 0.01 & LCOGT-1m \\
58089.829 & +89.6 & 14.51 & 0.01 & LCOGT-1m \\
58089.831 & +89.6 & 14.49 & 0.01 & LCOGT-1m \\
58090.800 & +90.6 & 14.57 & 0.07 & Asiago-Schmidt \\
58090.846 & +90.6 & 14.53 & 0.01 & LCOGT-1m \\
58090.848 & +90.6 & 14.52 & 0.01 & LCOGT-1m \\
58091.881 & +91.7 & 14.58 & 0.01 & LCOGT-1m \\
58091.883 & +91.7 & 14.59 & 0.01 & LCOGT-1m \\
58093.540 & +93.3 & 14.77 & 0.02 & NOT \\
58093.853 & +93.7 & 14.72 & 0.01 & LCOGT-1m \\
58093.855 & +93.7 & 14.67 & 0.01 & LCOGT-1m \\
58095.834 & +95.6 & 14.83 & 0.01 & LCOGT-1m \\
58095.836 & +95.6 & 14.83 & 0.01 & LCOGT-1m \\
58096.390 & +96.2 & 14.97 & 0.07 & Asiago-Schmidt \\
58096.820 & +96.6 & 14.89 & 0.01 & LCOGT-1m \\
58096.821 & +96.6 & 14.90 & 0.01 & LCOGT-1m \\
58097.169 & +97.0 & 14.98 & 0.01 & LCOGT-1m \\
58099.242 & +99.0 & 15.05 & 0.01 & LCOGT-1m \\
58099.244 & +99.0 & 15.12 & 0.01 & LCOGT-1m \\
58101.200 & +101.0 & 15.14 & 0.01 & LCOGT-1m \\
58101.202 & +101.0 & 15.13 & 0.01 & LCOGT-1m \\
58102.082 & +101.9 & 15.17 & 0.01 & LCOGT-1m \\
58102.084 & +101.9 & 15.17 & 0.01 & LCOGT-1m \\
58103.167 & +103.0 & 15.30 & 0.01 & LCOGT-1m \\
58103.169 & +103.0 & 15.32 & 0.01 & LCOGT-1m \\
58104.197 & +104.0 & 15.30 & 0.01 & LCOGT-1m \\
58104.199 & +104.0 & 15.32 & 0.01 & LCOGT-1m \\
58104.400 & +104.2 & 15.33 & 0.06 & Liverpool \\
58105.280 & +105.1 & 15.35 & 0.07 & Asiago-Schmidt \\
58105.844 & +105.6 & 15.28 & 0.01 & LCOGT-1m \\
58105.846 & +105.6 & 15.27 & 0.01 & LCOGT-1m \\
58109.340 & +109.1 & 15.45 & 0.06 & Asiago-Schmidt \\
58109.340 & +109.1 & 15.45 & 0.06 & Liverpool \\
58113.882 & +113.7 & 15.48 & 0.01 & LCOGT-1m \\
58113.885 & +113.7 & 15.49 & 0.01 & LCOGT-1m \\
58114.430 & +114.2 & 15.52 & 0.02 & Liverpool \\
58121.887 & +121.7 & 15.61 & 0.01 & LCOGT-1m \\
58121.889 & +121.7 & 15.60 & 0.01 & LCOGT-1m \\
58129.854 & +129.7 & 15.72 & 0.01 & LCOGT-1m \\
58129.857 & +129.7 & 15.74 & 0.01 & LCOGT-1m \\
58137.380 & +137.2 & 15.85 & 0.03 & NOT \\
58139.104 & +138.9 & 15.85 & 0.01 & LCOGT-1m \\
58139.107 & +138.9 & 15.86 & 0.01 & LCOGT-1m \\
58149.070 & +148.9 & 15.97 & 0.01 & LCOGT-1m \\
58149.073 & +148.9 & 15.96 & 0.01 & LCOGT-1m \\
58156.445 & +156.2 & 16.08 & 0.01 & LCOGT-1m \\
58156.448 & +156.2 & 16.08 & 0.01 & LCOGT-1m \\
58163.340 & +163.1 & 16.17 & 0.03 & NOT \\
58164.049 & +163.8 & 16.18 & 0.01 & LCOGT-1m \\
58164.052 & +163.8 & 16.23 & 0.01 & LCOGT-1m \\
\hline 
\multicolumn{5}{c}{$z$}\\
\hline 
58011.600 & +11.4 & 14.08 & 0.02 & NOT \\
58014.700 & +14.5 & 14.08 & 0.01 & NOT \\
58017.550 & +17.3 & 14.05 & 0.01 & NOT \\
58028.500 & +28.3 & 13.95 & 0.02 & Liverpool \\
58034.550 & +34.3 & 13.90 & 0.03 & Liverpool \\
58036.620 & +36.4 & 14.01 & 0.03 & NOT \\
58043.600 & +43.4 & 13.90 & 0.02 & Liverpool \\
58047.600 & +47.4 & 13.92 & 0.02 & NOT \\
58048.449 & +48.2 & 13.89 & 0.05 & Liverpool \\
58051.560 & +51.4 & 13.94 & 0.01 & NOT \\
58058.400 & +58.2 & 13.89 & 0.02 & Liverpool \\
58066.580 & +66.4 & 13.95 & 0.01 & NOT \\
58072.400 & +72.2 & 13.95 & 0.02 & Liverpool \\
58077.490 & +77.3 & 13.99 & 0.03 & Liverpool \\
58093.540 & +93.3 & 14.45 & 0.01 & NOT \\
58104.400 & +104.2 & 14.85 & 0.03 & Liverpool \\
58114.430 & +114.2 & 14.99 & 0.02 & Liverpool \\
58137.380 & +137.2 & 15.26 & 0.02 & NOT \\
58163.340 & +163.1 & 15.51 & 0.01 & NOT \\
\hline 
\enddata
\tablecomments{Phases are reported with respect to an assumed explosion epoch of MJD 57999.09}
\end{deluxetable}

